Transformer-VQ: Linear-Time Transformers via Vector Quantization

We introduce Transformer-VQ, a decoder-only transformer computing softmax-based dense self-attention in linear time. Transformer-VQ's efficient attention is enabled by vector-quantized keys and a novel caching mechanism. In our large-scale experiments, Transformer-VQ is shown highly competitive in quality, obtaining 0.99 bpb on Enwik8, 26.6 ppl on PG-19, and 3.16 bpb on ImageNet64. In addition, the optimized implementation of Transformer-VQ is over 3x faster than a comparable quadratic-time transformer at sequence length 8k, is over 12x faster at 32k, and can scale to 131k with similar throughput. Code available: \url{https://github.com/transformer-vq/transformer_vq}

==> intro.tex <==
\section{Introduction}

Transformer \citep{Vaswani2017} language models can easily scale to a few thousand sequence tokens, with their predictive abilities generally improving as context length increases \citep{ZDai2019, Kaplan2020}. In spite of the spectacular successes, the standard transformer uses a self-attention mechanism with a quadratic time complexity. This limits the practicality of applying transformers to even longer sequences due to a deterioration in processing speed. Transformer variants that overcome this limitation have the potential to improve a variety of applications and enable new breakthroughs. 

Up to this point, a variety of \emph{efficient transformers} \citep{YTay2020} have been proposed to scale to long sequences, generally with subquadratic or even linear complexity. Techniques include sparsity \citep{Child2019, Beltagy2020, Kitaev2020, Roy2021, Sukhbaatar2021, Wu2022, Liu2023}, compression \citep{Rae2020, CZhu2021, Ren2021}, low-rank approximations \citep{SWang2020, Katharopoulos2020, Xiong2021, Choromanski2021}, and cross-attention primitives \citep{XMa2021, Hutchins2022, Hawthorne2022}. Other parallelizable models for sequential data have also been proposed \citep{Zhai2021, AGu2022, LeeThorp2022, Peng2023, Poli2023}. 

In this paper, we propose Transformer-VQ, a transformer decoder with \emph{dense self-attention computible in linear time} with respect to sequence length. This is made possible through a combination of vector-quantized keys, localized positional biases, and a truncation-free cache mechanism. In addition, the model is fairly simple to implement and sample from. 

